Robust optimization for adversarial learning with finite sample complexity guarantees

Decision making and learning in the presence of uncertainty has attracted significant attention in view of the increasing need to achieve robust and reliable operations. In the case where uncertainty stems from the presence of adversarial attacks this need is becoming more prominent. In this paper we focus on linear and nonlinear classification problems and propose a novel adversarial training method for robust classifiers, inspired by Support Vector Machine (SVM) margins. We view robustness under a data driven lens, and derive finite sample complexity bounds for both linear and non-linear classifiers in binary and multi-class scenarios. Notably, our bounds match natural classifiers' complexity. Our algorithm minimizes a worst-case surrogate loss using Linear Programming (LP) and Second Order Cone Programming (SOCP) for linear and non-linear models. Numerical experiments on the benchmark MNIST and CIFAR10 datasets show our approach's comparable performance to state-of-the-art methods, without needing adversarial examples during training. Our work offers a comprehensive framework for enhancing binary linear and non-linear classifier robustness, embedding robustness in learning under the presence of adversaries.

==> chapters/old/old_introduction.tex <==
\section{Introduction}

Adversarial attacks in machine learning and deep models seem to be an inherent feature of these models. The study of adversarial attacks date back to classification models \cite{AML04} \cite{AML18c} and it gained much attention lately given the widespread use of neural networks. The academic literature is flourishing with adversarial examples \cite{AML04} \cite{AML13} \cite{AML14} \cite{AML18b} \cite{AML19} highlighting the tendency of ML models to learn superficial and brittle data statistics and hence presenting a security risk for models deployed in critical systems \cite{AML19b}. This poses a real treat since these models have been used in safety-critical applications such as autonomous driving \cite{AML16} \cite{AML17b}.

Limited-Memory BFGS (L-BFGS) \cite{AML13}, Fast Gradient Sign Method (FGSM) \cite{AML14}, Projected Gradient Descent (PGD) \cite{AML19c}, Carlini and Wagner (CW) \cite{AML17}, Jacobian-based Saliency Map Attack (JSMA) \cite{AML16d}, DeepFool (DF) \cite{DeepFool16} are just some of many adversarial generating procedures available in the literature. Several review papers, \cite{AML17b, AML18c, AdvTraining2021}, provide a summary and review state-of-the art attacks and defense procedures. 

That being said, several authors proposed different defense mechanisms against adversarial attacks. Defensive distillation \cite{AML16b} and feature squeezing \cite{AML18c} are some examples of techniques that proceed by reducing the dimension of the original model resulting in a more resilient model against adversarial attackers. Another approach, focused on the neural network space, proposes a new framework for training models \cite{AML14GAN} in which two neural networks (a classifier and an attacker) compete with each other in the form of a zero-sum game, where the attacker's gain is the classifier's loss.

These and other known successful defenses are effective to specific types of data tampering. However, these defenses provide empirical guarantees for one perturbation type and do not offer a good understanding of the guarantees they provide. This makes it difficult to navigate the landscape of adversarial robustness or to fully evaluate the possible security implications \cite{AML19c}.

It has been shown \cite{AML19b} that a trade-off in robustness to different types of perturbations must exist in a natural and simple statistical setting. Furthermore, the authors showed that models trained against multiple attacks fail to achieve robustness competitive with that of models trained on each attack individually.

In \cite{AML19c}, the authors study the adversarial robustness of neural networks through the lens of robust optimization. This formulation enables the authors to cast both attacks and defenses into a common theoretical framework, naturally encapsulating most prior work on adversarial examples.

\subsection{Summary of contributions}

\begin{itemize}
    \item Theoretically, we ...
    \item Algorithmically, we propose a data-driven-optimization adversarial-training procedure that ...
    \item Pratically, we ...
\end{itemize}

\subsection{Our methodology and results}


\subsection{Related work}




==> chapters/old/old_preliminaries.tex <==
\section{Preliminaries}

Let $\big(\Omega, \mathscr{F}, \mathcal{P} \big)$ be a probability
space, and
$\zeta: \big( \Omega, \mathscr{F} \big) \rightarrow \big( Z,
\mathscr{Z} \big)$ be a measurable map. Note that since $\zeta$ is
measurable one can define the measure induced by $\zeta$ or the
distribution of $\zeta$ as:

\[
 \mathbb{P}(z) = \big(\mathcal{P} \circ \zeta^{-1}\big) (z) = \mathcal{P}\big( \zeta^{-1}(z) \big), \forall z
  \in \mathscr{Z}
  \label{eqn:Pzeta}
\]

In addition, let $\mathcal{H}$ be a class of hypothesis or
models. Each $h \in \mathcal{H}$ is a function mapping
$ X \rightarrow Y$, where $X$ represents the the domain of features or
covariates and $Y$ the domain of response variables. This function is
also called a predictor, a hypothesis, or a classifier. In this case,
we can take $Z = X \times Y$ and $\zeta = [\chi, \upsilon]^T$.

We are concerned with the learning problem, in which the learner
wishes to find the best hypothesis $h$ that minimizes the risk
$\R{\mathbb{P}}{\ell(h(\chi), \upsilon)}$:

\begin{equation}
  \Opt{inf}{h \in \mathcal{H}}{\R{\mathbb{P}}{\ell(h(\chi), \upsilon)}}{}\label{Unc}
\end{equation}

where $\ell: Y \times Y \rightarrow \mathbb{R}_+$ is a loss function.

\subsection{Learning problem}

In a learning problem setup, the learner does not know the
distribution $\mathbb{P}$ but has access to $m$ independently
and identically distributed examples
$S = \big(z_1, \ldots, z_m\big) \in Z^m$, where each point
$z_i = (x_i, y_i)$ is sampled from to the fixed but unknown
distribution $\mathbb{P}$ of the random variable $\zeta$.

Note that the sample $S$ induces a probability in $Z^m$ which we
will denote by:

\begin{equation}
  \mathbb{P}^m(z) =  \mathbb{P} \times \ldots \times
  \mathbb{P}(z), \forall z \in \mathscr{Z} \times \ldots \times
  \mathscr{Z}
\end{equation}

In addition, the ``true'' risk or loss is not directly observed since
the learner does not know $\mathbb{P}$, but only has access to
$S$. Hence, the learner must resort to empirical risk
$\Remp{S}{\ell(h(x), y)}$ and work with measure concentration
inequalities to show convergence. We denote by $h_S^{ERM}$ the solution of
the of (\ref{Unc}) using the empirical risk minimization (ERM)
problem:
\begin{equation}
  h_S^{ERM} \in \Opt{argmin}{h \in \mathcal{H}}{\Eemp{\mathbb{P}}{\ell(h(x), y)}}{}\label{Uncemp}
\end{equation}

which can be simplified to:
\begin{equation}
  h_S^{ERM} = \Opt{argmin}{h \in \mathcal{H}}{\frac{1}{m}\sum_{i=1}^m{\ell(h(x_i), y_i)}}{}
\end{equation}

A successful learner should be able to progress from individual examples to broader generalization. This is also referred to as inductive reasoning or inductive inference. Formally speaking, the \emph{Probably Approximately Correct} (PAC) framework \cite{Book_ML_Mohri2018} defines the class of learnable concepts in terms of the number of samples needed to achieve an approximate solution and the computational complexity of the learning algorithm.

\begin{definition}
\label{def:PAC}
  \textbf{Agnostic PAC-learning} A hypothesis class $\mathcal{H}$ is   called agnostic PAC-learnable if there exists an algorithm $M$, that returns a hypothesis $h_S$ given the training sample $S$ and a polynomial function $p(.,.,. ,. )$ such that for any $\epsilon, \delta> 0$, \emph{for all distributions} $\mathcal{P}$ over $Z = X \times Y$, the following holds for any sample size $m \geq p(1/\epsilon, 1/\delta,dim(X))$ :

  \begin{equation}
    \mathcal{P}^m\Big(\E{\mathcal{P}}{\ell (h_S(\chi), \upsilon)} - \Opt{min}{h \in
      \mathcal{H}}{\E{\mathcal{P}}{\ell (h(\chi), \upsilon)}}{} \leq \epsilon \Big) \geq 1-\delta
  \end{equation}

  If $M$ further runs in $p(1/\epsilon, 1/\delta, dim(X))$, then it is said to be an \textbf{efficiently agnostic PAC-learning algorithm}.
\end{definition}

Note that the APAC framework is a distribution-free model: no particular assumption is made about the distribution $\mathcal{P}$. In fact, Additionally, the training sample and the test examples used to define the error are drawn according to the same distribution. This is a natural and necessary assumption for generalization to be possible in general \cite{Book_ML_Mohri2018}.

%Furthermore, by restricting the learner to choosing a predictor from
%$\mathcal{H}$, we bias it toward a particular set of predictors. Such
%restrictions are often called an inductive bias. Since the choice of
%such a restriction is determined before the learner sees the training
%data, it should ideally be based on some prior knowledge about the
%problem to be learned \cite{UnderstandingML14}. In fact, the excess
%error of a hypothesis $h \in \mathcal{H}$ can be decomposed as:
%\begin{equation}
%  R(h) - R^* = \underbrace{R(h) - \Opt{inf}{h \in \mathcal{H}}{R(h)}{}}_{\text{estimation}} +
%    \underbrace{\Opt{inf}{h \in \mathcal{H}}{R(h)}{} - R^*}_{\text{approximation}}
%\end{equation}

%where $R^*$ is the optimal minimizer over all measurable functions
%$h$. The PAC learning definition concentrates on bounding the
%estimation term.


\subsection{Adversarial attacks}

A common assumption \cite{Cullina2018, FeigeMansour2015, Madry2019,  LeeRaginsky2018, TuZhang2019} is that the adversary can tamper with the data as far as it is in the vicinity of the original example. More formally, $x^\prime \in N_\xi(x)$:

\begin{equation}
  N_\xi(x) := \Big\{x^\prime \Big| \norm{x^\prime-x} \le \xi \Big\}
\end{equation}

Consider now the following parametrized version of the ERM problem:
\begin{equation*}
  \Opt{min}
  {\theta \in \mathbb{R}^d}
  {\frac{1}{m}\sum_{i=1}^m{\ell(h_\theta(x_i), y_i)}}
  {}
\end{equation*}

\subsubsection*{Fast gradient sign method (FGSM)}
FGSM is an attack for an $\ell_\infty$-bounded adversary \cite{Goodfellow2015}
and computes an adversarial example as:
\begin{equation*}
x + \xi \cdot \text{sign}(\nabla_x \ell(h_\theta(x, y))
\end{equation*}

One interpretation is that this attack is a simple one-step scheme for
maximizing the inner part of the adversarial problem.

\subsubsection*{Projected gradient descent (PGD)}
A more powerfull attack \cite{Madry2019} is a multi-step variant of the FGSM:
\begin{equation*}
x_{t+1} = \Pi_{N_\xi(x)} (x_t + \eta \cdot \text{sign}(\nabla_x \ell(h_\theta(x, y)))
\end{equation*}

\subsubsection*{Carlini and Wagner (CW)}
This attack was proposed in \cite{Carlini2017} as a response to one approach
to defend against adversarial attacks.  
\begin{equation*}
  \Opt{min}
  {\xi}
  {\norm{\xi}_p + c f(x + \xi)}
  {x + \xi \in [0,1]^n}
\end{equation*}
The $\norm{.}_p$ measures the distance of the adversarial pertubation
and the function $f$ denotes a customized adversarial loss satisfying
$f(x + \xi) \leq 0$. The constraint $x + \xi \in [0,1]^n$ ensures
  that the image generated is a valid one.


\subsubsection*{DeepFool (DF)}
DeepFool is based on an iterative linearization of the classifier to
generate minimal perturbations that are sufficient to change
classification labels \cite{DeepFool2016}.  Specifically, at each
iteration, $h$ is linearized around the current point $x$ and the
minimal perturbation of the linearized classifier is computed as:
\begin{equation*}
  \Opt{min}
  {\xi}
  {\norm{\xi}_2}
  {h(x) + \nabla_f(x)^T \xi = 0}
\end{equation*}


\subsection{Adversarial defenses}

There are also several defense mechanisms against adversarial
attacks. Some of these are:

\begin{itemize}
\item Defensive distillation: The authors in \cite{Papernot2016} adapted the
  distillation procedure\footnote{ Distillation is a training
    procedure initially designed to train a neural network using
    knowledge transferred from a different neural network
    \cite{Papernot2016}} such that instead of using it to transferring
  knowledge between different architectures, they use the knowledge
  extracted from a neural network to improve its own resilience to
  adversarial samples.

\item Feature squeezing: In \cite{Xi2018}, the authors reduce the
  search space available to an adversary by coalescing samples that
  correspond to many different feature vectors in the original space
  into a single sample. By comparing a neural network model’s
  prediction on the original input with that on squeezed inputs,
  feature squeezing detects adversarial examples with high accuracy
  and few false positives.

\item Zero-sum game: Another approach, also focused on the neural
  network space, proposes a new framework for training models
  \cite{Goodfellow2014} in which two neural networks (a classifier and an
  attacker) compete with each other in the form of a zero-sum game,
  where the attacker's gain is the classifier's loss.

\item Adversarial training: Yet another defense mechanism is
  adversarial training \cite{Goodfellow2015, Madry2019, TRADES_ZhangElGhaoui2019}. It is
  considered to be one of the most effective approaches for deep
  learning models to defend against adversarial examples
  \cite{BaiTao2021}. Unlike other defense strategies, adversarial
  training aims to enhance the robustness of models intrinsically. The
  idea of adversarial training is straightforward: it augments
  training data with adversarial examples in each training loop. Thus
  adversarially trained models behave more normally when facing
  adversarial examples than stan- dardly trained models.
\end{itemize}


These and other known successful defenses are effective to specific
types of data tampering. However, these defenses provide empirical
guarantees for one perturbation type and do not offer a good
understanding of the guarantees they provide. This makes it difficult
to navigate the landscape of adversarial robustness or to fully
evaluate the possible security implications \cite{Madry2019}.


It has been shown \cite{Tramer2019} that a trade-off in robustness to
different types of perturbations must exist in a natural and simple
statistical setting. Furthermore, the authors showed that models
trained against multiple attacks fail to achieve robustness
competitive with that of models trained on each attack individually.


In \cite{Madry2019}, the authors study the adversarial robustness of neural
networks through the lens of robust optimization. This formulation
enables the authors to cast both attacks and defenses into a common
theoretical framework, naturally encapsulating most prior work on
adversarial examples.


\cite{AMLCrypto19b} followed a different path and considered the
possibility that adversarial attacks do always exist. Their results
indicate that perhaps a similar approach to cryptography (relying on
computational hardness) holds promise for achieving computationally
robust machine learning.


In the robust optimization framework, the assumption is that the
decision maker has very little knowledge about the underlying
distribution. The key idea is to define an uncertainty set of possible
realizations unknown parameters. The decision-maker then proceeds by
optimizing the worst-case cost over this uncertainty set
\cite{ElGhaoui1997} \cite{ElGhaoui1998} \cite{BenTalNemirovski1998}
\cite{BenTalNemirovski2000} \cite{Book_BenTalElGhaoui2009}.

\subsection{Adversarial training}

Our primary interest is to analyze the adversarial training in the PAC
learning framework. As described in \cite{BaiTao2021},
adversarial training is one of the most effective approaches for deep
learning models to defend against adversarial examples. Unlike other
defense strategies, adversarial training aims to enhance the
robustness of models intrinsically.

The authors in \cite{Szegedy2014, Goodfellow2015} pointed out that standard
supervised training does not specify that the chosen function be
resistant to adversarial examples. They argue that this must be
encoded in the training procedure given the evidence that a neural
network could be regularized by training on a mixture of adversarial
and clean examples. One interpretation \cite{Goodfellow2015} of this
adversarial training procedure is that the learner is leaning by
playing an adversarial game, or learning by minimizing an upper bound
on the expected cost over noisy samples. It can also be seen as a form
of active learning, where the model is able to request labels on new
points \cite{Goodfellow2015}. They proceed by training with an adversarial
objective function based on the fast gradient sign method, whereas the
authors in \cite{Madry2019} propose a multi-step variant, which is
essentially projected gradient descent on the negative loss function.

A common assumption \cite{Cullina2018, FeigeMansour2015, Madry2019,
  LeeRaginsky2018, TuZhang2019} is that the adversary can
tamper with the data as far as it is in the vicinity of the original
example. More formally, $g(x) \in N_\xi(x)$:

\begin{equation}
  N_\xi(x) := \Big\{x^\prime \Big| \norm{x^\prime-x} \le \xi \Big\}
\end{equation}

Furthermore, the authors in \cite{Madry2019} propose the adversarial
empirical risk minimization (AERM) paradigm to reliably train models
that are robust to adversarial attacks. They continue by proposing a
concrete guarantee that an adversarially robust model should satisfy
and then adapt the training methods towards achieving this
guarantee. More precisely, they analyse the following parametrized
saddle point problem:

\begin{equation}
  \Opt{min}
  {\theta}
  {\E{\mathbb{P}}{\Opt{max}{x \in N_\xi(x)}{\ell(\theta, x, y)}{}}}
  {}
\end{equation}


\subsubsection*{Example: Linear regression}

Consider now the hypothesis class of linear functionals,
$\mathcal{H} = \{h_{a, b}: x \rightarrow a^T x + b \ \big| \ a \in
\mathbb{R}^d, b \in \mathbb{R} \}$. The learner whishes to find
$a,b$ that solves the following:

\begin{align*}
  &\Opt{min}{a,b \in R^{d+1}}{\frac{1}{2}{\E{\mathbb{P}}{\norm{y - (a^Tx + b)}_2^2}}}{}
\end{align*}

To train against adversarial attacks the learner considers the robust
counterpart of the above problem. This is refered to adversarial risk
minimization in the literature:

\begin{align*}
  &\Opt{min}
    {a, b \in R^{d+1}}
    {\E{\mathbb{P}}{\Opt{max}
    {\delta}
    {\frac{1}{2}\norm{y - (a^T(x + \delta) + b)}_2^2}
    {\norm{\delta} \leq \xi}}}
    {}
\end{align*}


\textbf{ERM}
Given samples
$ S = \big((x_1, y_1), \ldots, (x_m, y_m)\big)$ the
learner proceeds by finding $a, b$ that minimizes the quadratic
empirical loss:

\begin{align*}
  &\Opt{min}{a,b \in R^d}{\frac{1}{2m}\sum_{i=1}^m{\norm{y_i - (a^Tx_i + b)}_2^2}}{}
\end{align*}

One approach to solving this optimization problem is to rely on
gradient descent methods. Yet, an alternative is to use OLS
procedure. For this, let us fist write the problem in matrix form:
\begin{equation*}
  \Opt{min}{\theta \in R^d}{\frac{1}{2m}{\norm{Y - X \theta}_2^2}}{}
\end{equation*}

with $\theta = [a^T, b]^T$, $Y = [y_1, \ldots, y_m]^T$ and
$X = [[x_1^T, 1], \ldots, [x_m^T, 1]]^T$.

Through OLS the optimizal solution is:
\begin{equation*}
  \theta^*  =
  \left\{
    \begin{aligned}
      (X^TX)^{-1}X^TY \  &\text{, if } X^TX \text{ is invertible}\\
      (X^TX)^\dagger X^TY \  &\text{, otherwise}
  \end{aligned}
  \right.
\end{equation*}

\textbf{AERM}

\begin{equation*}
  \Opt{min}
  {a, b\in \mathbb{R}^{d+1}}
  {\frac{1}{m}\sum_{i=1}^m
    \Opt{max}
      {\delta \in \mathbb{R}^d} 
      {\norm{y_i - (a^T(x_i+ \delta) + b)}_2^2}
      {\norm{\delta} \leq \xi}}
  {}
\end{equation*}

The optimal $\delta^*$ that solves the inner maximization problem is
the solution of either:
\begin{equation*}
  \left\{
    \begin{aligned}
    \Opt{max}
      {\delta \in \mathbb{R}^d} 
      {y_i - (a^T(x_i+ \delta) + b)}
      {\norm{\delta} \leq \xi}\\
          \Opt{min}
      {\delta \in \mathbb{R}^d} 
      {y_i - (a^T(x_i+ \delta) + b)}
      {\norm{\delta} \leq \xi}
    \end{aligned}
    \right.
  \end{equation*}

and solving this is equivalent to solving the following problems:
\begin{equation*}
  y_i - (a^Tx_i + b) +\left\{
     \begin{aligned}
     \Opt{max}
      {\delta \in \mathbb{R}^d} 
      {-a^T \delta}
      {\norm{\delta} \leq \xi} \\
    \Opt{min}
      {\delta \in \mathbb{R}^d} 
      {-a^T \delta}
      {\norm{\delta} \leq \xi}
    \end{aligned}
    \right.
\end{equation*}

given the definition of the dual norm,
$\norm{y}_* = \Opt{sup}{x}{y^Tx}{\norm{x} \leq 1}$, the above can be
rewritten as:
\begin{equation*}
  y_i - (a^Tx_i + b) +\left\{
    \begin{aligned}
      \xi \norm{a}_* \\
      -\xi \norm{a}_*
    \end{aligned}
    \right.
  \end{equation*}

or, in a simple form:
  
\begin{equation*}
  y_i - (a^Tx_i + b) -\xi \norm{a}_*
\end{equation*}

As a result, the AERM becomes:

\begin{equation*}
  \Opt{min}
  {a, b \in \mathbb{R}^d}
  {\frac{1}{m}\sum_{i=1}^m
  \norm{y_i - (a^Tx_i + b + \xi \norm{a}_*)}_2^2}
  {}
\end{equation*}


\subsubsection*{Example: logistic binary classifier}

In this case $y \in \{0,1\}$. We will be working wiht the class of
logistic regression models
$\mathcal{H} = \{h_{a, b}: x \rightarrow 1/(1 + e^{-(a^T x + b)}) \
\big| \ a \in \mathbb{R}^d, b \in \mathbb{R} \}$.


\textbf{ERM}

In this case the learner whishes to find $a,b$ that minimizes the
cross entropy:

\begin{align*}
  &\Opt{min}{a,b \in R^{d+1}}{\E{\mathbb{P}}{-y \log\Big( \frac{1}{1 + e^{-(a^T x + b)}}\Big) -(1-y) \log\Big( 1- \frac{1}{1 + e^{-(a^T x + b)}}  \Big)}}{}\\
  &\Opt{min}{a,b \in R^{d+1}}{\E{\mathbb{P}}{y \log( 1 + e^{-(a^T x + b)} ) + (1-y) \log( 1 + e^{(a^T x + b)} )}}{} \\
\end{align*}

and its robust counterparty:

\begin{equation*}
  \Opt{min}
    {a,b \in \mathbb{R}^{d+1}}
    {\E{\mathbb{P}}
      {\Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {y \log( 1 + e^{-(a^T (x + \delta) + b)} ) + (1-y) \log( 1 + e^{(a^T (x + \delta) + b)} )}
        {\norm{\delta} \leq \xi }}}
    {}
\end{equation*}


\textbf{AERM}

\begin{equation*}
  \Opt{min}
    {a,b \in \mathbb{R}^{d+1}}
    {\frac{1}{m}\sum_{i=1}^m
      \Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {y_i \log( 1 + e^{-(a^T (x_i + \delta) + b)} ) + (1-y_i) \log( 1 + e^{(a^T (x_i + \delta) + b)} )}
        {\norm{\delta} \leq \xi }}
    {}
\end{equation*}

Let us focus first on the inner maximization problem:
\begin{equation*}
\Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {y_i \log( 1 + e^{-(a^T (x_i + \delta) + b)} ) + (1-y_i) \log( 1 + e^{a^T (x_i + \delta) + b} )}
        {\norm{\delta} \leq \xi }
\end{equation*}
 

If $y_i = 1$, the maximixation can be simplified to: 
\begin{equation*}
      \Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {\log( 1 + e^{-(a^T (x_i + \delta) + b)} )}
        {\norm{\delta} \leq \xi }
\end{equation*}


The objective function in this case is monotonically decreasing,
finding $\delta$ that solves the maximization is equivalent to
finding $\delta$ that solves:
\begin{align*}
  &\Opt{min}
        {\delta \in \mathbb{R}^{d}}
        {a^T (x_i + \delta) + b}
        {\norm{\delta} \leq \xi } \\
  &a^Tx_i + b + \Opt{min}
        {\delta \in \mathbb{R}^{d}}
        {a^T \delta}
        {\norm{\delta} \leq \xi } \\
\end{align*}

By the definition of the dual norm, $\norm{y}_* = \Opt{sup}{x}{y^Tx}{\norm{x} \leq 1}$:
\begin{equation*}
  \Opt{min}
        {\delta \in \mathbb{R}^{d}}
        {a^T \delta}
        {\norm{\delta} \leq \xi } = -\xi \norm{a}_* 
\end{equation*}

The maximizaiton becomes:
\begin{equation*}
      \Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {\log( 1 + e^{-(a^T (x_i + \delta) + b)} )}
        {\norm{\delta} \leq \xi } =
      \log(1 + e^{-(a^T x_i + b + \xi \norm{a}_*)})
\end{equation*}

Now, if $y_i = 0$:
\begin{equation*}
      \Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {\log( 1 + e^{a^T (x_i + \delta) + b} )}
        {\norm{\delta} \leq \xi }
\end{equation*}

In this case, the objective function is monotonically increasing,
and proceeding on a similar manner, leads to solving:
\begin{align*}
    &\Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {a^T (x_i + \delta) + b}
        {\norm{\delta} \leq \xi } \\
  &a^Tx_i + b + \Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {a^T \delta}
        {\norm{\delta} \leq \xi } \\
\end{align*}

And The maximizaiton becomes:
\begin{equation*}
      \Opt{max}
        {\delta \in \mathbb{R}^{d}}
        {\log( 1 + e^{a^T (x_i + \delta) + b} )}
        {\norm{\delta} \leq \xi } =
      \log(1 + e^{a^T x_i + b + \xi \norm{a}_*})
\end{equation*}

Finally, the simplified form of the AERM is:
\begin{equation*}
  \Opt{min}
    {a,b \in \mathbb{R}^{d+1}}
    {\frac{1}{m}\sum_{i=1}^m
        y_i \log( 1 + e^{-(a^T x_i + b + \xi \norm{a}_*)} ) + (1-y_i) \log( 1 + e^{a^T x_i + b + \xi \norm{a}_*} )}
    {}
\end{equation*}


